Incorporating Bias-aware Margins into Contrastive Loss for Collaborative Filtering

Collaborative filtering (CF) models easily suffer from popularity bias, which makes recommendation deviate from users' actual preferences. However, most current debiasing strategies are prone to playing a trade-off game between head and tail performance, thus inevitably degrading the overall recommendation accuracy. To reduce the negative impact of popularity bias on CF models, we incorporate Bias-aware margins into Contrastive loss and propose a simple yet effective BC Loss, where the margin tailors quantitatively to the bias degree of each user-item interaction. We investigate the geometric interpretation of BC loss, then further visualize and theoretically prove that it simultaneously learns better head and tail representations by encouraging the compactness of similar users/items and enlarging the dispersion of dissimilar users/items. Over eight benchmark datasets, we use BC loss to optimize two high-performing CF models. On various evaluation settings (i.e., imbalanced/balanced, temporal split, fully-observed unbiased, tail/head test evaluations), BC loss outperforms the state-of-the-art debiasing and non-debiasing methods with remarkable improvements. Considering the theoretical guarantee and empirical success of BC loss, we advocate using it not just as a debiasing strategy, but also as a standard loss in recommender models.

==> backup/0_abstract.tex <==
\begin{abstract}
Collaborative filtering models are well known to suffer from popularity bias, which causes the recommendations to deviate from users' actual interests. 
However, most current debiasing strategies only promote the rankings of low-popularity items, failing to fundamentally enhance discriminative power by learning better representations. 
It inevitably results in degrading the overall recommendation utility. 

In this paper, we propose bias-margin contrastive loss (BC Loss), a variant of softmax loss, to learn highly discriminative representations that pull positive samples together while push negative samples at least a bias-dependent angular margin apart.
Geometrically, BC loss can be viewed as imposing angular margin on a hypersphere manifold.
The size of the angular margin can be quantitatively adjusted by the popularity bias degree. 
We investigate the clear geometric interpretation of BC loss and analytically prove that BC loss simultaneously encourages similar user/item compactness and enlarges dissimilar user/item dispersion. 
These two properties clearly show the reason why BC loss benefits discriminative representation learning and generalization capability of the model.
We validate our proposed BC loss on Matrix Factorization (MF) and LightGCN, which are representative of the conventional and SOTA backbone models for collaborative filtering. 
Extensive experiments over two backbone models on four real-world datasets demonstrate that BC loss outperforms both debiasing and non-debiasing methods with remarkable improvements in both imbalanced and balanced evaluations. 
Considering the theoretical guarantee and empirical success of BC loss, we recommend using BC loss not only as a debiasing technique but also a general choice of the objective function in recommender system.
We will release our implementation upon acceptance.
\end{abstract}

==> backup/1_introduction.tex <==
\section{Introduction}
% 1.TODO: Background of CF: representation learning; long-tail; narrow down to popularity bias will lead to biased representations.

The core task of Collaborative Filtering (CF) in recommendation is learning the representations of users and items from historical interactions, such that the cosine or Euclidean distance between two representations reflects their semantic similarity. 
However, one of the main challenges in learning high-quality representations in CF is the popularity bias issues in data \cite{unfairness,Crowd,MostPop,Beyond_Parity}.
Typically, the training data distribution is usually long-tailed, \eg a few head items occupy most of the interactions, whereas the majority of tail items are unpopular and receive relatively little attention.
Due to this imbalanced property of the training data, the resultant CF model will inherit the popularity bias and, in many cases, amplify the bias by over-recommending the head items and under-recommending the tail items. 
As a result, the popularity bias is causing the biased representations with poor generalization ability, leading the recommendations to deviate from users' actual interests.


% 2.TODO: Related works: Limitations & Motivations
Motivated by the existence of such biases, popularity debiasing methods that aim to lift the tail performance have been studied extensively. 
Unfortunately, most prevalent debiasing techniques focus on the trade-off between the head and tail evaluations, \eg post-processing re-ranking \cite{Calibration,RankALS,rescale,FPC,PC_Reg}, balanced training loss \cite{ESAM,ALS+Reg,Regularized_Optimization,PC_Reg}, sample re-weighting \cite{ips,IPS-C,IPS-CN,Propensity_SVM-Rank,YangCXWBE18,UBPR}, and head bias removal by causal inference \cite{CausE,PDA,DecRS,MACR}. 
Worse still, many of them hold the assumptions that are infeasible in reality, \eg the balanced test distribution is known in advance to guide the hyperparameters adjustment \cite{DICE, MACR}, and a small unbiased subset data is existent for training unbiased model \cite{KDCRec,CausE}. 
Consequently, these methods encounter the difficulty that tail performance rise sacrifices the head performance and leads to a severe overall performance drop.
We argue that the head and tail trade-off results in low-quality representations, which hardly improve the generalization ability of debiasing models.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/intro.pdf}
    \vspace{-5pt}
    \caption{Illustration of separative and discriminative representations. Dots represent item representations, while star refers to the user representation. Positive and negative samples are in red and blue, respectively.}
    \label{fig:intro}
    \vspace{-15pt}
\end{figure}

% 3.TODO: a. Recommendation needs discriminative; b. Discriminative power characterizes; c. Softmax loss limitation.
We conjecture that a debiased model truly improves long-tailed performance in CF by learning better user/item representations, but not by playing a head and tail performance trade-off. 
For the recommendation task, the user/item is required to be mapped into not only separable but also discriminative representation space,
since it is impractical to pre-collect all the users' positive responses.
Taking an implicit-feedback recommender as an example, it only leverages positive user-item interactions, such as clicks, to learn personalized user preferences, and the lack of such clicks does not indicate a negative response from the users.
Such a positive-unlabeled problem asks the learned representations to be discriminative and generalized enough to predict users' preferences without true labels.
The two critical properties for discriminative representations are high compactness for positive samples and large dispersion for negative samples, as shown in Figure \ref{fig:intro}.  % Lack references
However, the softmax loss \cite{softmax} only encourage the separability to preserve maximal information \cite{alignment_uniformity}.

% 4.TODO: a. Purpose: generalize the softmax: better representations, better long-tail performance; b. specifically, ... c. pull & push
The purpose of this paper, therefore, is to modify the softmax loss to a more general and highly efficient BC loss, short for Bias-margin Contrastive loss, to obtain discriminative representations in the recommendation task.
Specifically, we impose an interaction-wise bias-dependent angular margin between every positive user/item pair and negative samples.
The size of the angular margin can be quantitatively controlled by a bias degree extractor.
If the user-item pair's popularity bias degree is low, which means it is a hard example, we further add a larger margin to strongly squeeze the tightness of those under-represented samples (usually inactivated users with tail items) to improve generalization. 
In contrast, when the value of bias degree extractor is high, \eg user-item interactions can be correctly predicted using only popularity information of user-item pair, we adjust the softmax loss by no margin or smaller margin to reduce the importance of these biased examples (in most cases, some head user-item pairs).
By optimizing BC loss, the user/item representations become more discriminative by pulling positive representations together and pushing negative representations apart.
As a result, BC loss can significantly improve both head and tail performance.

% 5.TODO: a.clear geometric interpretation; b.hard example mining strategy; c. Analytical proof 
The BC loss has several desirable advantages.
First, it has a clear and intuitive geometric interpretation, as elaborated in Figure \ref{fig:intro}.
From a geometric view, we impose a popularity bias-related margin on a hypersphere manifold to enlarge dissimilar representations' distance.
Second, the interaction-wise adaptive margin forces the optimization to concentrate on the hard examples, a simple but efficient hard example mining strategy. 
The implicit effect of the hard example mining strategy is to encourage the model to shift its attention to more informative hard samples instead of relying on biased samples.
Third, theoretical analysis in Section 2 reveals that BC loss tends to learn a low-entropy cluster for positive samples (\eg high similar item/user compactness) and a high-entropy feature space (\eg large dissimilar item/user dispersion). 
In this case, BC loss benefits alleviate the popularity bias as well as the general recommendation task.


% 6. Contribution: a. A new solution to debias problem; b. BC loss; c.effectiveness, use as a general loss in CF.
Our main contributions can be summarized as follows.
\begin{itemize}[leftmargin=*]
\item To the best of our knowledge, we are among the first to reduce the popularity bias in CF by enhancing the discriminative power of the loss function.
\item We devise a generalized softmax loss - BC loss, equipped with an intuitive geometric interpretation, an efficient hard example mining strategy, and a clear theoretical analysis.
\item Promising results demonstrate that BC loss not only alleviates popularity bias amplification effectively but also improves both head and tail performance in both imbalanced and balanced evaluations.
\end{itemize}
BC loss opens up the possibility of constructing a highly discriminative loss function for the traditional recommendation.
Considering the theoretical guarantee and empirical effectiveness of BC loss, we recommend using BC loss not only as a debiasing technique but also as a standard loss in CF.









==> backup/2_methodology.tex <==
\section{Methodology}

% 1.TODO: Detailed Methodology

The personalized item recommendation is usually based on implicit feedback \cite{softmax} whose goal is to retrieve a subset of interesting items for a given user from a large catalog of items.
We consider the standard formulation of implicit feedback recommendation as a top-n ranking problem.
Given a historical interaction dataset $\Set{O}^{+}=\{(u,i)|y_{ui}=1\}$ with $u \in \Space{U}$ a user, $i \in \Space{I}$ an item, and $y_{ui}$ indicating the user $u$ has adopted item $i$ before, a scoring function $\hat{y}: \Space{U}\times \Space{I} \rightarrow \Space{R}$ is optimized to reflect the preference of the user for the item. 

For a single user-item pair, recommender utilizes an item encoder $\phi: \Space{I} \rightarrow \Space{R}^d$, a user encoder $\psi: \Space{U} \rightarrow \Space{R}^d$, and a similarity function $s: \Space{R}^d \times \Space{R}^d \rightarrow \Space{R}$. 
These functions are composed as follows: 
\begin{equation*}
    \hat{y}(u,i) = s(\psi(u), \phi(i))
\end{equation*}
The choice of item/user encoder, the backbone of the recommender, can be roughly categorized into ID-based (\eg MF \cite{BPR,SVD++}, NMF \cite{NMF}, CMN \cite{cmn}), history-based (\eg SVD++ \cite{SVD++}, FISM \cite{FISM}, MultVAE \cite{MultVAE}), and graph-based models (\eg NGCF \cite{NGCF}, PinSage \cite{PinSage}, LightGCN \cite{LightGCN}). 
Moreover, the design of similarity function $s(\dot)$ can be dot product, cosine similarity, or more complex multilayer perceptron (MLP) \cite{NMF}.

To the end, we conduct our experiments in the representative of the conventional backbone MF and the SOTA backbone LightGCN. 
Furthermore, a cosine similarity is used as the similarity function, suggested in \cite{RendleKZA20}, for better interpretation, which is denoted as
\begin{equation*}
    s(\psi(u), \phi(i))=\frac{<\psi(u), \phi(i)>}{\norm{\psi(u)} \cdot \norm{\phi(i)}} 	\doteq \cos{(\hat{\theta}_{ui})}
\end{equation*}
in which $\hat{\theta}_{ui}$ is the angle between the representation of a user $\psi(u)$ and an item $\phi(i)$.

\textbf{Classical Learning Strategy.}
The classical learning strategy of collaborative filtering (CF) model can be classified into three groups: point-wise loss (\eg binary cross-entropy \cite{CrossEntropy}, mean square error \cite{SVD++}), pair-wise loss (\eg BPR \cite{BPR}, WARP \cite{WARP}) and softmax loss \cite{softmax}. 
Point-wise and pair-wise loss are long-standing and most-used objective functions in CF. 
However, large-scale studies theoretically and empirically confirm that both point-wise and pair-wise losses will inevitably propagate more information towards head user-item pairs, which causes gradient shifts and amplifies popularity bias \cite{PC_Reg,unfairness,tang2020investigating}. 
On the other hand, recent years have witnessed a growing academic interest in using softmax loss in recommender systems \cite{sgl,CLRec,S3-Rec}, due to its wide success in self-supervised contrastive learning. 

Hence, in this paper, we set sampled softmax loss as the learning objective and minimize it to train the parameters over a dataset of size $|\Set{O}^{+}|$:
\begin{gather*}
    \min\Lapl_0 = -\sum_{(u,i)\in\Set{O}^{+}}\log\frac{\exp{(\cos(\hat{\theta}_{ui})/\tau)}}{\exp{(\cos(\hat{\theta}_{ui})/\tau)}+\sum_{j\in\Set{N}_{u}}\exp{(\cos(\hat{\theta}_{uj})/\tau)}}
\end{gather*}
where $(u,i)\in\Set{O}^{+}$ is one observed interaction of user $u$, while $\Set{N}_{u}=\{j|y_{uj}=0\}$ is the sampled unobserved items that $u$ did not interact with before; $\tau$ is the hyper-parameter known as the temperature in softmax \cite{tau}. 

Although, softmax loss has been outstandingly successful in various fields due to its inherent property of alignment, which assigns similar features to cohere together \cite{alignment,WuXYL18}. 
Softmax loss, as a widespread self-supervised representation learning loss, encourages the learned features uniformly distributed to preserve maximal information for helping downstream tasks \cite{alignment_uniformity,SaunshiPAKK19}. 
Unfortunately, the modification of softmax loss to enhance discriminative representation as well as reduce the popularity bias has seldomly been studied. 
Therefore, the goal of this paper is to conduct a more generic and broadly applicable variant of softmax loss in CF tasks, which can fundamentally improve the long-tail performance in CF.  

\subsection{Bias-Margin Contrastive Loss}

\textbf{Popularity bias extractor.} 
How do we know if an example exhibits popularity bias? 
How could we quantify the degree of popularity bias for a single user-item pair?
Although it is impractical to directly measure the distribution shift without accessing the test data, CF models are unlikely to predict well, given only biased information.
Specifically, the biased information could be user popularity statistics $p_u \in \Space{P}$, the number of historical items that user $u$ interacted with before, and the item popularity statistics $p_i \in \Space{P}$, the number of observed interactions that item $i$ is involved in. 
If the CF models could still correctly predict the user's preference using only $p_u$ and $p_i$, it is likely due to CF models learning the popularity bias.
Moreover, the extent of the prediction recovery will capture the degree of popularity bias.

Similarly as a standard CF model, the popularity bias extractor can be formalized as a function $\hat{y}_b: \Space{P}\times \Space{P} \rightarrow \Space{R}$ and composed of an item popularity encoder $\phi_b:\Space{P} \rightarrow \Space{R}_d$, a user popularity encoder $\psi_b: \Space{P} \rightarrow \Space{R}^d$, and a cosine similarity function $s: \Space{R}^d \times \Space{R}^d \rightarrow \Space{R}$, which is defined as
\begin{equation*}
    \hat{y}_b(p_u,p_i) = s(\psi_b(p_u), \phi_b(p_i)) \doteq cos(\hat{\xi}_{ui})
\end{equation*}
in which $\hat{\xi}_{ui}$ is the angle between the user popularity embedding $\psi_b(p_u)$ and item popularity embedding $\phi_b(p_i)$.

The popularity bias extractor $\hat{y}_b$ can be trained using sampled softmax loss $\Lapl_b$:
\begin{gather} \label{equ:bias_extractor}
    \min\Lapl_b = -\sum_{(u,i)\in\Set{O}^{+}}\log\frac{\exp{(\cos(\hat{\xi}_{ui})/\tau)}}{\exp{(\cos(\hat{\xi}_{ui})/\tau)}+\sum_{j\in\Set{N}_{u}}\exp{(\cos(\hat{\xi}_{uj})/\tau)}}
\end{gather}

This optimization forces the popularity bias extractor  $\hat{y}_b$  to reconstruct the historical interaction and assess the popularity degree from an interaction perspective.
Those interactions that can not be predicted well using only popularity statistics are hard examples, which are more informative for representation learning.
In other words, the popularity bias extractor is helpful to identify the hard examples in the training set and carefully measures how hard it is for each user-item pair.

\textbf{Bias-margin Contrastive Loss (BC loss).} 
Instead of designing a weighted combination of softmax loss and a popularity bias penalty, we propose a more elegant way to learn discriminative representations by adding popularity bias-related angular margin.
Our Bias-margin Contrastive Loss (BC loss) is formulated as:
\begin{gather}\label{equ:bc_loss}
    \Lapl_{BC} = -\sum_{(u,i)\in\Set{O}^{+}}\log\frac{\exp{(\cos(\hat{\theta}_{ui}+M_{ui})/\tau)}}{\exp{(\cos(\hat{\theta}_{ui}+M_{ui})/\tau)}+\sum_{j\in\Set{N}_{u}}\exp{(\cos(\hat{\theta}_{uj})/\tau)}}
\end{gather}

Where $M_{ui}$ is the interaction-wise additive angular margin corresponding to user $u$ and item $i$. 

With larger $M_{ui}$, the additive angular margin becomes larger and the learning objective becomes harder.
Intuitive, we prefer larger angular margin for the hard example, which helps the CF model concentrates on the hard examples to compensate biases, more detailed illustrations in Section \ref{sec:three_advantages}.

In this study, we constrain the margin in a popularity bias view:
\begin{gather}
    M_{ui} = \min \{\hat{\xi}_{ui}, \pi - \hat{\theta}_{ui}\}
\end{gather}
Where the purpose of the upper bound $\pi - \hat{\theta}_{ui}$ is to restrict the $\cos(\hat{\theta}_{ui} + \cdot)$ to be a monotonically decreasing function corresponding to the angular margin. 

The choice of bias-margin $M_{ui}$ is various. 
A series of margin selections, such as $M_{ui} = \min\{\lambda \cdot \hat{\xi}_{ui}, \pi - \hat{\theta}_{ui}\}$, is also reasonable, where $\lambda$ controls the strength of the bias-margin.
Meanwhile, by carefully constructing a monotonically decreasing similarity function, we can get ride of the restriction: $\pi - \hat{\theta}_{ui}$.
However, Such modifications are heuristic-based, and come at the price of increased complexity or additional hyper-parameters.
We encourage the reader to further explore, but will not list and compare them in this article.

BC loss is extremely easy to implement in recommendation task, which only needs revise several lines of code. 
Moreover, BC loss only adds negligible computational complexity during training compared with softmax loss, but achieves better representations as clearly shown in Section \ref{sec:three_advantages} and \ref{sec:toy_example}. 
Hence, we recommend using BC loss not only as a debiasing technique but also as a standard loss in recommender system.


\subsection{Three Advantages of BC Loss} \label{sec:three_advantages}
Our proposed BC loss has three advantages: an intuitive geometric interpretation, a novel hard example mining strategy, and clear theoretical properties.

\textbf{Geometric Interpretation.}
We firstly revisit the softmax loss by looking its ranking criteria. To simplify the geometric interpretation, we analyze one user $u$ with one positive item $i$ and only two negative items $j_1, j_2$. Then the posterior probabilities obtained by softmax loss are:
\begin{gather*}
    \frac{\exp{(\cos(\hat{\theta}_{ui})/\tau)}}{\exp{(\cos(\hat{\theta}_{ui})/\tau)}+\exp{(\cos(\hat{\theta}_{uj_1})/\tau)}+\exp{(\cos(\hat{\theta}_{uj_2})/\tau)}}
\end{gather*}

\begin{figure}[t]
	\centering
	\subcaptionbox{Softmax Loss (2D)\label{fig:2d_softmax}}{
	    \vspace{-5pt}
		\includegraphics[width=0.38\linewidth]{figures/2d-softmax.pdf}}
	\subcaptionbox{BC Loss (2D)\label{fig:2d_bc}}{
	    \vspace{-5pt}
		\includegraphics[width=0.38\linewidth]{figures/2d-bc.pdf}}
	\subcaptionbox{Softmax Loss (3D)\label{fig:3d_softmax}}{
	    \vspace{-5pt}
		\includegraphics[width=0.38\linewidth]{figures/3d-softmax.pdf}}
	\subcaptionbox{BC Loss (3D)\label{fig:3d_bc}}{
	    \vspace{-5pt}
		\includegraphics[width=0.38\linewidth]{figures/3d-bc.pdf}}
	\vspace{-10pt}
	\caption{Geometric Interpretation of softmax loss and BC loss. The first row is the 2D hypersphere manifold for user representation constraint, and the second row is the 3D constraint. The dark red region indicates the discriminative user constraint for each loss, while the light red region is for comparison.}
	\label{fig:geometric_interpretation}
	\vspace{-13pt}
\end{figure}


In the training stage, the softmax loss requires $\hat{\theta}_{ui} > \hat{\theta}_{uj_1}, \hat{\theta}_{ui} > \hat{\theta}_{uj_2}$ to model the basic assumption in recommendation task.
Concretely, if an item $i$ has been viewed by user $u$, then we assume that the user $u$ prefers the item $i$ over all other non-observed items $j_1,j_2$. 
We will skip the analysis for BPR loss since the constraint and geometric interpretation can be easily obtained by considering one negative item.

What if we add an angular margin to making the criteria more stringent? Intuitively, we instead requires $\hat{\theta}_{ui} + M_{ui} > \hat{\theta}_{uj_1}, \hat{\theta}_{ui} + M_{ui} > \hat{\theta}_{uj_2}$ where $M_{ui}$ is a bias-related value. By directly formulating this idea into the modified softmax loss, we have the posterior probabilities for BC loss, similar in Equation \eqref{equ:bc_loss}:

\begin{gather*}
    \frac{\exp{(\cos(\hat{\theta}_{ui}+ M_{ui})/\tau)}}{\exp{(\cos(\hat{\theta}_{ui}+M_{ui})/\tau)}+\exp{(\cos(\hat{\theta}_{uj_1})/\tau)}+\exp{(\cos(\hat{\theta}_{uj_2})/\tau)}}
\end{gather*}
We can see that BC loss is more rigor about the ranking assumption. More detailed explanations of assumption are given in Section \ref{sec:hard_example}. 

The comparison of geometric interpretation for softmax loss and BC loss is depicted in Figure \ref{fig:geometric_interpretation}. 
Assume the learned items $i,j_1,j_2$ are given, and softmax and BC losses are optimized to the same value.
The constraint boundaries for correctly ranking the user's preference in Softmax are $\hat{\theta}_{ui} = \hat{\theta}_{uj_1}, \hat{\theta}_{ui} = \hat{\theta}_{uj_2}$, while in BC loss, the constraint boundaries are $\hat{\theta}_{ui} + M_{ui} = \hat{\theta}_{uj_1}, \hat{\theta}_{ui} + M_{ui} = \hat{\theta}_{uj_2}$.
Geometrically, from softmax loss to BC loss, it is a more stringent circle-like region on the unit sphere in the 3D case, as illustrated in Figure \ref{fig:3d_bc}.
Note that a larger bias-related margin $M_{ui}$ leads to a smaller hypercycle-like region, which is an explicit discriminative constraint on a manifold.
Limited constraint regions squeeze the tightness of similar items, at the same time, enlarge the dissimilar item's distance.
As the dimension of representations increases, BC loss has more difficult learning objective requirements, which exponentially decreases the area of constraint regions for correct ranking.
Consequently, BC loss is gradually powerful to learn discriminative representations in recommendation tasks.



\textbf{Hard Example Mining Strategy.} \label{sec:hard_example}
We argue that BC loss naturally inherits the idea of hard example mining to improve training efficiency and effectiveness. 

The key for hard example mining strategy is to mine the most valuable samples.
The popularity bias extractor $\hat{y}_b$, defined in Equation \eqref{equ:bias_extractor}, can be viewed as a hard example detector.
If the value of popularity bias is high, which means the interaction could be predicted by using only popularity information, then the corresponding user-item pair is a biased sample.
In most cases, those biased samples are activated users with famous items.
Take a news recommender system as an example; the reader is possible to click the news only because it is a top story, not because its topic is a long-term interest for that reader. 
Here, the bias-related margin $M_{ui}$ is close to zero.
In other words, we still make the basic assumption that the reader favors the popular news over all other unobserved news.

In contrast, the popularity bias extractor identifies the hard examples when the popularity statistics can not successfully predict the interactions.
Those user-item pairs, in general, are inactivated users with unpopular items.
Recall the news recommendation example; the reader clicking a piece of niche news is more likely to be attracted by interesting keywords or specific news topics.  
Those interactions are of importance in helping the recommendation model understand user behavior.
Specifically, the bias margin $M_{ui}$ is significant in this situation, and we assume a more stringent assumption that the reader prefers this unpopular news by a large margin to other unclicked news.
The large margin makes the objective function more challenging to learn. 
As a result, leading the model shifts its attention to hard examples.


\textbf{Theoretical Properties of BC Loss.}
We show that BC loss has compactness part and dispersion part on representation learning based on the following theorem.

\begin{theorem}
Assuming the representations of users and items are normalized, then minimizing the BC loss is equivalent to simultaneously minimizing a compactness part and a dispersion part:
\begin{align*}
    \Lapl_{BC} &  \propto \underbrace{\sum_{u=1}^{|\Space{U}|}\norm{\Mat{v}_u-\Mat{c}_u}^2 + \sum_{i=1}^{|\Space{I}|}\norm{\Mat{v}_i-\Mat{c}_i}^2}_{\text{Compactness part}}\underbrace{-\sum_{u=1}^{|\Space{U}|}\sum_{j\in\Set{N}_{u}}\norm{\Mat{v}_u-\Mat{v}_j}}_{\text{Dispersion part}} \\
    & \propto \underbrace{\mathcal{H}(\Mat{V}|Y)}_{\text{Compactness}}\:\: \underbrace{- \:\: \mathcal{H}(\Mat{V})}_{\text{Dispersion}}\: = \:- \mathcal{I}(\Mat{V};Y)
\end{align*}
\end{theorem}

\begin{proof}
Throughout this section, for simplicity, $\Mat{v}_u \doteq \psi(u)$ and $\Mat{v}_i \doteq \phi(i)$. 
We use the upper-case letter $\Mat{V} \in \Space{V}$ to indicate the random vector of representation, where $\Space{V} \subseteq \Space{R}^d$ is the representation space.
We also use the normalization assumption for representations to connect cosine and Euclidean distances, \ie if $\norm{\Mat{v}_u}=1, \forall u$ and $\norm{\Mat{v}_i}=1, \forall i$, then $\Mat{v}_u^T\Mat{v}_i = 1 - \frac{1}{2} \norm{\Mat{v}_u-\Mat{v}_i}^2$. 

It is clear that we can find a upper bound $m$, \st $-1 < \cos(\hat{\theta}_{ui}+M_{ui}) \leq \Mat{v}_u^T\Mat{v}_i - m <  1 $. 
Let $\Set{P}_u = \{i|y_{ui} =1\}$ denotes the positive items set for user $u$, $\Set{P}_i = \{u|y_{ui} =1\}$ refers to the positive user set for item $i$, and $\Set{N}_{u}=\{i|y_{ui}=0\}$ represents the negative items set for user $u$.
Let us start by splitting the BC loss into two terms:
\begin{align} 
    \Lapl_{BC} & \geq  -\sum_{(u,i)\in\Set{O}^{+}}\log\frac{\exp{\{(\Mat{v}_u^T\Mat{v}_i - m)/\tau}\}}{\exp{\{(\Mat{v}_u^T\Mat{v}_i - m)/\tau\}}+\sum_{j\in\Set{N}_{u}}\exp{\{(\Mat{v}_u^T\Mat{v}_j)/\tau\}}} \nonumber\\
    & = -\sum_{u=1}^{|\Space{U}|}\sum_{i \in \Set{P}_u} \frac{\Mat{v}_u^T\Mat{v}_i - m}{\tau} \nonumber\\
    & + \sum_{u=1}^{|\Space{U}|}\sum_{i \in \Set{P}_u} \log \{\exp{\{\frac{\Mat{v}_u^T\Mat{v}_i - m}{\tau}\}}+\sum_{j\in\Set{N}_{u}}\exp{\{\frac{\Mat{v}_u^T\Mat{v}_j}{\tau}\}}\} \label{eq:split_bc}
\end{align}

Let $\Mat{c}_{u} = \frac{1}{|\Set{P}_u|}\sum_{i\in \Set{P}_{u}}\Mat{v}_i$ denotes the hard mean of all items in the positive items set for user $u$. 
Similarly, let $\Mat{c}_{i} = \frac{1}{\Set{P}_{i}} \sum_{u\in\Set{P}_{i}} \Mat{v}_{u}$. 
Let the symbol $\eqc$ indicates equality up to a multiplicative and/or additive constant. 
We first analyze the first term in Equation \eqref{eq:split_bc} by illustrating it to a compactness term of the center loss.
\begin{align}
    -\sum_{u=1}^{|\Space{U}|}\sum_{i \in \Set{P}_u} \frac{\Mat{v}_u^T\Mat{v}_i - m}{\tau} 
    & =  \sum_{u=1}^{|\Space{U}|}\sum_{i \in \Set{P}_u} \frac{\norm{\Mat{v}_u-\Mat{v}_i}^2}{2\tau} +\frac{m-1}{\tau} \nonumber\\
    & \eqc \sum_{u=1}^{|\Space{U}|}\sum_{i \in \Set{P}_u} \norm{\Mat{v}_u-\Mat{v}_i}^2 \nonumber\\
    & = \sum_{u=1}^{|\Space{U}|}\sum_{i \in \Set{P}_u} (\norm{\Mat{v}_u}^2 + \norm{\Mat{v}_i}^2 - 2\Mat{v}_u^T\Mat{v}_i)\nonumber\\
    & = \sum_{u=1}^{|\Space{U}|}\sum_{i \in \Set{P}_u} (\norm{\Mat{v}_u}^2 - \Mat{v}_u^T\Mat{v}_i )
    + \sum_{i=1}^{|\Space{I}|}\sum_{u\in\Set{P}_i} (\norm{\Mat{v}_i}^2 - \Mat{v}_u^T\Mat{v}_i )\nonumber \\
    & \eqc \sum_{u=1}^{|\Space{U}|}\norm{\Mat{v}_u-\Mat{c}_u}^2 + \sum_{i=1}^{|\Space{I}|}\norm{\Mat{v}_i-\Mat{c}_i}^2 \label{eq:conpactness}
\end{align}
where we use the properties of normalization in the first line and the definitions of $\Mat{c}_i$ and $\Mat{c}_u$ in the last line. 
Note that, we technically link the K-means to the first term of our BC loss in Equation \eqref{eq:split_bc}. 

Combining the two term in Equation \eqref{eq:conpactness}, we obtain:
\begin{align*}
    -\sum_{(u,i)\in\Set{O}^{+}}\frac{\Mat{v}_u^T\Mat{v}_i - m}{\tau} \eqc \sum_{\Mat{v}\in \Space{V}} \norm{\Mat{v} - \Mat{c}_{v}}^2
\end{align*}

Following \cite{BoudiafRZGPPA20}, we can then interpret the first term in Equation \eqref{eq:split_bc} as a conditional cross-entropy between $\Mat{V}$ and another random variable $\bar{\Mat{V}}$, whose conditional distribution given $Y$ is a standard Gaussian $\bar{\Mat{V}}|Y \sim \mathcal{N}(\Mat{c}_{\Mat{V}},I)$:
\begin{align}
    -\sum_{(u,i)\in\Set{O}^{+}}\frac{\Mat{v}_u^T\Mat{v}_i - m}{\tau} & \eqc
    \mathcal{H}(\Mat{V};\bar{\Mat{V}}|Y)=\mathcal{H}(\Mat{V}|Y)+\mathcal{D}_{KL}(\Mat{V}||\bar{\Mat{V}|Y}) \nonumber\\
    & \propto \mathcal{H}(\Mat{V}|Y) \label{eq:first-term}
\end{align}
As a consequence, minimizing the first term in Equation \eqref{eq:split_bc} is equivalent to minimizing $\mathcal{H}(\Mat{V}|Y)$.
This concludes the proof for the first compactness part of BC loss.

We then analyze the second term in Equation \eqref{eq:split_bc} to demonstrate its dispersion property:
\begin{align}
 & \sum_{u=1}^{|\Space{U}|}\sum_{i \in \Set{P}_u} \log \{\exp{\{\frac{\Mat{v}_u^T\Mat{v}_i - m}{\tau}\}}+\sum_{j\in\Set{N}_{u}}\exp{\{(\frac{\Mat{v}_u^T\Mat{v}_j}{\tau}\}}\}\nonumber\\
 & \geq \sum_{u=1}^{|\Space{U}|}\sum_{i \in \Set{P}_u} \log{(
 \sum_{j\in\Set{N}_{u}}\exp{\{\frac{\Mat{v}_u^T\Mat{v}_j}{\tau}\}})} \nonumber\\
 & \geq \sum_{u=1}^{|\Space{U}|}\sum_{j\in\Set{N}_{u}}\exp{\{\frac{\Mat{v}_u^T\Mat{v}_j}{\tau}\}}\nonumber\\
 & \eqc - \sum_{u=1}^{|\Space{U}|}\sum_{j\in\Set{N}_{u}} \norm{\Mat{v}_u - \Mat{v}_j}^2 \label{eq:dispersion}
\end{align}
Where we drop the redundant term with the compactness objective in the second line, and use the Jensen's inequality in the third line. Following \cite{WangS11}, the negative of term in Equation \eqref{eq:dispersion} is the entropy estimator $\hat{\mathcal{H}}(\Mat{V})$. Then, we know that minimizing the second term in Equation \eqref{eq:split_bc} is equivalent to maximizing $\mathcal{H}(\Mat{V})$:
\begin{align} \label{eq:second-term}
         \sum_{u=1}^{|\Space{U}|}\sum_{i \in \Set{P}_u} \log \{\exp{\{\frac{\Mat{v}_u^T\Mat{v}_i - m}{\tau}\}}+\sum_{j\in\Set{N}_{u}}\exp{\{\frac{\Mat{v}_u^T\Mat{v}_j}{\tau}\}}\} \propto -\mathcal{H}(\Mat{V})
\end{align}
Combining Equation \eqref{eq:first-term} and \eqref{eq:second-term}, we conclude the proof.
\end{proof}

\textbf{Discussion.}
The BC loss breaks down into a compactness part and a dispersion part.
For the compactness part, $\Mat{c}_{u}$ is the mean of all items that user $u$ has interaction with, which is a simple representation for the interest of user $u$.
Moreover, $\Mat{c}_{i}$ denotes the hard mean of all users in the positive users set for item $i$, which is the most straightforward portrait of all users who love item $i$.
In other words, the compactness part of BC loss encourages each user to be close to his interests while each item is tight to the portrait of all users who interact with the specific item.
From the entropy view, the compactness part of BC loss tends to learn a low-entropy cluster for positive samples, \ie high similar item/user compactness.
On the other hand, the dispersion part of BC loss maximizes the pair-wise euclidean distance for negative samples, which is equivalent to forcing negative samples to stand far apart from one another.
From the entropy view, the dispersion part enforces the spread of representations to learn a high-entropy representation space \ie large dissimilar user/item separation degree. 






\subsection{Visualization of A Toy Experiment} \label{sec:toy_example}

\begin{figure*}[t]
	\centering
	\subcaptionbox{BPR loss for (head)\label{fig:head_bpr}}{
	    \vspace{-5pt}
		\includegraphics[width=0.24\linewidth]{figures/head_bpr.pdf}}
	\subcaptionbox{Softmax loss (head)\label{fig:head_softmax}}{
	    \vspace{-5pt}
		\includegraphics[width=0.24\linewidth]{figures/head_info.pdf}}
	\subcaptionbox{BC loss (head)\label{fig:head_bc}}{
	    \vspace{-5pt}
		\includegraphics[width=0.24\linewidth]{figures/head_bc.pdf}}
	\subcaptionbox{IPS-CN\cite{IPS-CN} (head) \label{fig:head_ips}}{
	    \vspace{-5pt}
		\includegraphics[width=0.24\linewidth]{figures/head_ips.pdf}}
	\subcaptionbox{BPR loss (tail)\label{fig:tail_bpr}}{
	    \vspace{-5pt}
		\includegraphics[width=0.24\linewidth]{figures/tail_bpr.pdf}}
	\subcaptionbox{Softmax loss (tail)\label{fig:tail_softmax}}{
	    \vspace{-5pt}
		\includegraphics[width=0.24\linewidth]{figures/tail_info.pdf}}
	\subcaptionbox{BC loss (tail)\label{fig:tail_bc}}{
	    \vspace{-5pt}
		\includegraphics[width=0.24\linewidth]{figures/tail_bc.pdf}}
	\subcaptionbox{IPS-CN\cite{IPS-CN} (tail)\label{fig:tail_ips}}{
	    \vspace{-5pt}
		\includegraphics[width=0.24\linewidth]{figures/tail_ips.pdf}}
	\vspace{-5pt}
	\caption{Visualization of item representations learned with different loss functions on Yelp2018. The identical head/tail user and the selected 500 items are drawn in (a-d)/(e-h). The first row of each subfigure shows the 3D item representations projected on the unit sphere. The second row of each subfigure shows the angle distribution of both positive and negative items for the specific head/tail user. 
	BC loss encourages the majority positive items to fall into the group closest to the user and further achieves the smallest mean positive angle.
	Some item representations are almost clustered at one point by learning BC loss.
	Moreover, only BC loss shows a 0.5-radian margin for the tail user between positive and negative samples.
	These phenomena verify that, compared to training with other loss functions, the BC loss simultaneously encourages similar user/item compactness and enlarges dissimilar user/item dispersion, strongly enhancing discriminative power for a better recommendation.}
	\label{fig:toy-example}
	\vspace{-8pt}
\end{figure*}

To intuitively visualize the effect of BC loss in recommendation task, a toy example on Yelp2018 \cite{LightGCN} dataset is presented.
We modify the two-layer LightGCN by reducing the output number of the last hidden layer to three, which means the dimension of the representations is three. 
So we can directly normalize the obtained 3-dimensional representations and plot them on a 3D unit sphere for visualization in Figure \ref{fig:toy-example}.
We train the recommendation models with identical lightGCN backbone over the training dataset by minimizing different loss functions.
For the same head or tail user (green star), we plot 500 items' representations in the unit sphere containing all positive items (red dots) and randomly selected negative items (blue dots) from both training and testing sets. 
The angle distribution (the second row of each subfigure) of positive and negative samples for a specific user quantitatively shows the discriminative power of each losses. 
We observe that:

\begin{itemize}[leftmargin = *]
    \item \textbf{In both head and tail user cases, BC loss learns more discriminative representations.} 
    As Figures \ref{fig:head_bc} and \ref{fig:tail_bc} show, for head and tail users, BC loss encourages around 40\% and 50\% of positive items to fall into the group closest to user representations, respectively. 
    In other words, the representations of those samples are almost clustered at one point.
    BC loss also achieves the smallest distance \wrt mean positive angle.
    This verifies that BC loss tends to learn a high similar item/user compactness.
    Moreover, a 0.5-radian margin is clearly shown in Figure \ref{fig:tail_bc} between positive items and negative items, reflecting a highly discriminative power.
    We conjecture that, compared with softmax loss performance in Figures \ref{fig:head_softmax} and \ref{fig:tail_softmax}, the compactness and dispersion properties of BC loss come from the incorporating of interaction-wise popularity bias-related margin.
    
    \item \textbf{The representations learned by BPR and Softmax losses are not discriminative enough.}
    Under the supervision of BPR and Softmax losses, the item representations are separably allocated in a wide range of the unit sphere, where blue and red points occupy almost the same space area, demonstrated in Figures \ref{fig:head_bpr} and \ref{fig:tail_softmax}.
    Furthermore, it seems only a negligible overlapping for angle distribution of positive and negative samples in Figure \ref{fig:tail_bpr}.
    However, because the number of positive and negative items is likely to be more than ten times different for the tail user, a small overlap will cause a large number of negative items to rank in front of positive items, significantly destroying the accuracy of recommendation.
    Consequently, it is not satisfactory to directly use BPR and softmax losses for the task of personalized recommendation.
    
    \item \textbf{The IPS-CN, a well-known popularity debiasing method in CF, is prone to lift the tail performance by sacrificing the representation learning for the head.}
    Compared with BPR loss in Figure \ref{fig:tail_bpr}, IPS-CN learns better item representations for the tail user, which only a slight part of distribution overlap for positive and negative samples, illustrated in Figure \ref{fig:tail_ips}.
    However, for the head user in Figure \ref{fig:head_ips}, the positive and negative item representations are mixed in a large space and cannot distinguish between each other.
    This results in a huge performance drop for head evaluations; more results can be found in Experiments.
\end{itemize}














==> chapters/0_abstract_new.tex <==
\begin{abstract}

Collaborative filtering (CF) models easily suffer from popularity bias, which makes recommendation deviate from users' actual preferences.
However, most current debiasing strategies only promote the rankings of low-popularity items, rather than learning better representations to fundamentally enhance the discriminative power and generalization ability of model.
\wx{They tend to trade-off between the head and tail performance, inevitably resulting in the degradation of the overall recommendation accuracy.}
% It causes the trade-off between head and tail performance, thus inevitably degrading the overall recommendation utility.

To learn powerful representations, we propose a \underline{B}ias-margin \underline{C}ontrastive loss (\textbf{BC Loss}) to train \wx{the} CF models, which pulls positive user-item pairs together, while pushing negative pairs apart to produce a bias-aware angular margin.
Geometrically, BC loss imposes the angular margin on a hypersphere manifold, which quantitatively tailors to the popularity bias degree of a user-item interaction.
We investigate the geometric interpretation of BC loss, and further theoretically prove that BC loss simultaneously encourages the compactness of similar users/items, and enlarges the dispersion of dissimilar users/items.
It clearly explains why BC loss learns bias-aware angularly discriminative representations, and endows the CF models with better discriminative power and generalization ability.
We use BC loss to optimize two high-performing CF models (MF \cite{BPR}, LightGCN \cite{LightGCN}) over four benchmark datasets.
On both imbalanced and balanced test evaluations, BC loss outperforms the state-of-the-art debiasing and non-debiasing methods with remarkable improvements.
Considering the theoretical guarantee and empirical success of BC loss, we recommend \wx{the use of} BC loss not only as a debiasing technique, but also as a general choice of the objective function in recommender models.
\wx{Codes and datasets are available at \url{https://anonymous.4open.science/r/BC-Loss-9DF2}.}
% We will release our implementation upon acceptance.




\end{abstract}

==> chapters/7_checklist.tex <==
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{This paper proposes a novel debiasing algorithm for recommendation system, which does not have any negative societal impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix~\ref{sec:proof}.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include code by URL in abstract.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix~\ref{sec:implementation}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{sec:implementation}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

